Using the Web as an Implicit Training Set: Application to Noun Compound Syntax and Semantics

An important characteristic of English written text is the abundance of noun compounds - sequences of nouns acting as a single noun, e.g., colon cancer tumor suppressor protein. While eventually mastered by domain experts, their interpretation poses a major challenge for automated analysis. Understanding noun compounds' syntax and semantics is important for many natural language applications, including question answering, machine translation, information retrieval, and information extraction. I address the problem of noun compounds syntax by means of novel, highly accurate unsupervised and lightly supervised algorithms using the Web as a corpus and search engines as interfaces to that corpus. Traditionally the Web has been viewed as a source of page hit counts, used as an estimate for n-gram word frequencies. I extend this approach by introducing novel surface features and paraphrases, which yield state-of-the-art results for the task of noun compound bracketing. I also show how these kinds of features can be applied to other structural ambiguity problems, like prepositional phrase attachment and noun phrase coordination. I address noun compound semantics by automatically generating paraphrasing verbs and prepositions that make explicit the hidden semantic relations between the nouns in a noun compound. I also demonstrate how these paraphrasing verbs can be used to solve various relational similarity problems, and how paraphrasing noun compounds can improve machine translation.

==> pst-jftree.tex <==
% 10 January 2004, John Frampton (frampton@neu.edu)
% Users should feel free to modify this file in any way they
% see fit.  If these modification go beyond your personal
% use, please send me a careful description of the
% modifications that have been made and the reasons that
% they were made.
% 13 Jan, 2004 - error message if no root node defined in \jftree

\csname JFTreeLoaded\endcsname
\let\JFTreeLoaded\endinput
\ifx\PSTricksLoaded\endinput \else \input pstricks \fi\relax
\ifx\PSTnodesLoaded\endinput \else \input pst-node \fi\relax
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
%%%%%%%%%%%%%%%%%%%%%%%
%% register resources
\newtoks\jfteverynode
\newdimen\jft@xpos
\newdimen\jft@ypos
\newdimen\m@xl
\newdimen\m@xr
\newdimen\m@xb
\newbox\jft@treebox
%%%%%%%%%%%%%%%%%%%%%%%
%% new PSTricks parameters
\def\psset@nodetopgap#1{\pssetlength\pst@dima{#1}%
   \edef\n@detopgap{\the\pst@dima}}
\def\psset@nodebotgap#1{\pssetlength\pst@dima{#1}%
   \edef\n@debotgap{\the\pst@dima}}
\def\psset@everynode#1{\jfteverynode={#1}}
\def\psset@triratio#1{\edef\jft@triratio{#1}}
\def\psset@scaleby#1{\edef\jft@scaleby{#1}}
%%%%%%%%%%%%%%%%%%%%%%%

\def\jftpsset#1{\ifx#1\relax\relax
   \else \psset{#1}\fi \ignorespaces}
\def\jftpsset#1{\edef\temp{#1}\ifx\temp\@empty
   \else \expandafter\psset\expandafter{\temp}\fi \ignorespaces}

%
\def\jft@getpars#1{\def\k@@p{#1}\futurelet\temp\jft@getparsA}
\def\jft@getparsA{\ifx\temp[\let\next\jft@getparsB
   \else \def\jft@pars{}\let\next=\k@@p \fi\next}
\def\jft@getparsB[#1]{\def\jft@pars{#1}\k@@p}
%\jft@getparsC}
%\def\jft@getparsC{\futurelet\temp\jft@getparsD}
%\def\jft@getparsD{\k@@p}

% define a branch
\def\defbranch{\jft@getpars\d@fbranch}
\def\d@fbranch#1#2(#3)#4(#5){%
   \edef#1{\noexpand\bgroup
      \edef\noexpand\@hleg{#5}%
      \edef\noexpand\@vleg{#3}%
      \edef\noexpand\m@kelevelpars{\jft@pars}%
      \noexpand\jft@getpars\noexpand\dr@wbranch}}
\def\dr@wbranch{\jftpsset{\m@kelevelpars}
   {\jftpsset{\jft@pars}
   \pssetxlength\pst@dima{\@vleg}
   \pst@dima=-\jft@scaleby\pst@dima
   \@scalebyslope\pst@dima{\@hleg}\pst@dima
   \edef\@hleg{\the\pst@dima}%
   \pssetylength\pst@dima{\@vleg}
   \pst@dima=\jft@scaleby\pst@dima
   \edef\@vleg{\the\pst@dima}%
   \pst@dima=\jft@xpos \pst@dimb=\jft@ypos
   \advance\jft@xpos by \@hleg
   \advance\jft@ypos by -\@vleg
   \psline(\pst@dima,\pst@dimb)(\jft@xpos,\jft@ypos)
   \xdef\temp{\noexpand\jft@xpos=\the\jft@xpos
      \noexpand\jft@ypos=\the\jft@ypos}%
   \aftergroup\temp}%
   \ev@ltarget}
%
\def\ev@ltarget{\futurelet\temp\ev@ltargetA}
\def\ev@ltargetA{\ifx\temp\bgroup\let\next\ev@ltargetB \else
   \let\next\ev@ltargetC \fi \next}
\def\ev@ltargetB#1{\setbox0=\hbox{{\jft@testnode #1}}%
   \d@@fnode \setn@de \egroup\ignorespaces}
\def\ev@ltargetC#1{#1\egroup\ignorespaces}

% use \@scalebyslope\pst@dima{3/4}\pst@dimb
%   \pst@dima is the height to be scaled,
%   the result is put in \pst@dimb
\def\@scalebyslope#1#2#3{#3=#1\expandafter
   \@@scalebyslope\expandafter#3#2//}
\def\@@scalebyslope#1#2/#3/{\pst@divide{#1}{#2pt}\temp
   #1=\temp pt \def\temp{#3}%
   \ifx\temp\@empty \let\next=\relax
      \else \multiply#1 by #3 \let\next=\@gobble\fi \next}

\def\deftriangle{\jft@getpars\d@ftriangle}
\def\d@ftriangle#1#2(#3)#4(#5)#6(#7){%
   \edef#1{\noexpand\bgroup
      \edef\noexpand\@leftleg{#5}%
      \edef\noexpand\@rightleg{#7}%
      \edef\noexpand\@upleg{#3}%
      \edef\noexpand\m@kelevelpars{\jft@pars}%
      \noexpand\jft@getpars\noexpand\dr@wtriangle}}
\def\dr@wtriangle{\jftpsset{\m@kelevelpars}
   {\jftpsset{\jft@pars}
   \pssetxlength\pst@dima{\@upleg}
   \pst@dima=\jft@scaleby\pst@dima
   \pst@dimb=-\pst@dima
   \@scalebyslope\pst@dima{\@leftleg}\pst@dima
   \@scalebyslope\pst@dimb{\@rightleg}\pst@dimb
   \edef\@leftleg{\the\pst@dima}%
   \edef\@rightleg{\the\pst@dimb}%
   \pssetylength\pst@dima{\@upleg}
   \pst@dima=\jft@scaleby\pst@dima
   \edef\@upleg{\the\pst@dima}%
   \pst@dima=\jft@xpos \pst@dimb=\jft@ypos  % save old
   \pst@dimc=\jft@xpos \advance\pst@dimc by \@rightleg % right edge
   \advance\jft@xpos by -\@leftleg   % left edge
   \advance\jft@ypos by -\@upleg     % new bottom edge
   \pspolygon(\jft@xpos,\jft@ypos)(\pst@dimc,\jft@ypos)(\pst@dima,\pst@dimb)
   \ifdim\pst@dimc>\m@xr \global\m@xr=\pst@dimc \fi
   \ifdim\jft@xpos<\m@xl \global\m@xl=\jft@xpos \fi
   \pst@dimc=\@leftleg \advance\pst@dimc by \@rightleg
   \xdef\jfttriwd{\the\pst@dimc}%
   \advance\jft@xpos by \jft@triratio\pst@dimc
   \xdef\temp{\noexpand\jft@xpos=\the\jft@xpos
      \noexpand\jft@ypos=\the\jft@ypos
      \noexpand\def\noexpand\jfttriwd{\the\pst@dimc}}%
   \aftergroup\temp}%
   \ev@ltarget}
\def\triline#1{\hbox to\jfttriwd{#1}}

% define a variable width triangle
\def\defvartriangle{\jft@getpars\d@fvartriangle}
\def\d@fvartriangle#1#2(#3){%
   \edef#1{\noexpand\bgroup
      \edef\noexpand\@upleg{#3}%
      \edef\noexpand\m@kelevelpars{\jft@pars}%
      \noexpand\jft@getpars\noexpand\dr@wvartriangle}}
\def\dr@wvartriangle#1{\jftpsset{\m@kelevelpars}
   \jftpsset{\jft@pars}
   \setbox0=\hbox{{\jft@testnode #1}}%
   \pst@dima=\jft@xpos \pst@dimb=\jft@ypos  % save old
   \advance\jft@xpos by -\jft@triratio\wd0
   \pst@dimc=\jft@xpos
   \advance\pst@dimc by \wd0
   \pssetylength\pst@dimd{\@upleg}
   \pst@dimd=\jft@scaleby\pst@dimd
   \advance\jft@ypos by -\pst@dimd
   \pspolygon(\jft@xpos,\jft@ypos)(\pst@dimc,\jft@ypos)(\pst@dima,\pst@dimb)
   \ifdim\pst@dimc>\m@xr \global\m@xr=\pst@dimc \fi
   \ifdim\jft@xpos<\m@xl \global\m@xl=\jft@xpos \fi
   \advance\jft@xpos by .5\wd0
   \d@@fnode \setn@de \egroup}

% disposition of the {stuff} associated with a node
\def\d@fnode#1#2#3\cr{%
   \if@rootnode \def\@startnode{#1}\@rootnodefalse\fi
   \def#1{%
   \setbox0=\hbox{{\jft@testnode #2}}%
   \d@@fnode
   \def\temp{#1}\ifx\temp\@startnode
      \xdef\adj@stht{-\the\jft@ypos}\fi
   \setn@de #3}}
\def\d@@fnode{%
   \ifn@degaps \else  \pssetylength\pst@dimg{\n@detopgap}
      \advance\jft@ypos by -\pst@dimg \fi
   {\advance\jft@xpos by-.5\wd0
      \ifdim\jft@xpos<\m@xl \global\m@xl=\jft@xpos \fi
    \advance\jft@xpos by\wd0
      \ifdim\jft@xpos>\m@xr \global\m@xr=\jft@xpos \fi}%
   \advance\jft@ypos by -\ht0}
\def\setn@de{%
   \pst@dima=-\dp0
   \rput[B](\jft@xpos,\jft@ypos){\copy0}
   \advance\jft@ypos by\pst@dima
   \ifdim\jft@ypos<\m@xb \global\m@xb=\jft@ypos \fi
   \ifn@degaps \else \pssetlength\pst@dimg{\n@debotgap}
      \advance\jft@ypos by -\pst@dimg \fi \ignorespaces}

% look for \omit and take appropriate action
\newif\ifn@degaps
\def\jft@testnode{\futurelet\temp\jft@testn@de}
\def\jft@testn@de{\ifx\temp\omit
      \global\n@degapstrue \let\next=\@gobble
   \else \global\n@degapsfalse
      \edef\next{\the\jfteverynode}\fi \next}

\newif\if@rootnode
\def\jftree{\jft@getpars\jft@tree}
\def\jft@tree{\setbox\jft@treebox=\hbox\bgroup \let\!=\d@fnode
   \let\@startnode=\@empty
   \jftpsset{\jft@pars}
   \jft@xpos=0pt \jft@ypos=0pt \m@xl=0pt \m@xr=0pt \m@xb=0pt
   \@rootnodetrue
   \ignorespaces}
\def\endjftree{\ifx\@startnode\@empty
   \errmessage{JFTree Error: Root node definition is missing}\fi
   \@startnode\egroup
   \dp\jft@treebox=-\m@xb
   \leavevmode\kern-\m@xl\raise\adj@stht\box\jft@treebox\kern\m@xr}

\let\defnode=\d@fnode

%% set defaults
\newpsstyle{jftreedefault}{arrows=c-c,linewidth=.6pt,scaleby=1,
   nodetopgap=3pt,nodebotgap=3pt,triratio=.5,everynode=\strut}
\psset{style=jftreedefault}
%% provide a minimal complement of branches and triangles
\defbranch\medleft(1)(1)
\defbranch\medright(1)(-1)
\defbranch\medvert(1)(1/0)
\deftriangle\medtri(1)(1)(-1)
\defvartriangle\medvar(1)

\catcode`\@=\TheAtCode\relax
\endinput


